Lower Gravity Demonstratable Testbed for Space Robot Experiments

In developing mobile robots for exploration on the planetary surface, it is crucial to evaluate the robot's performance, demonstrating the harsh environment in which the robot will actually be deployed. Repeatable experiments in a controlled testing environment that can reproduce various terrain and gravitational conditions are essential. This paper presents the development of a minimal and space-saving indoor testbed, which can simulate steep slopes, uneven terrain, and lower gravity, employing a three-dimensional target tracking mechanism (active xy and passive z) with a counterweight.

==> macrosForEThesis.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   macrosForEThesis.tex
%%   -------------------
%%
%%   Title: LaTeX macro file for the English Thesis
%%   
%%   
%%   Belief:
%%   1."Fig. 1: ~~~", "Table 1: ~~~" are for the figure and table citation.
%%   2. add the config to read the source code file (hello.c) and visualize it. 
%%
%%   Change Log:
%%   2020.11.26 Initial creation by Kentaro UNO
%%
%%   Contact:
%%   Please contact the author Kentaro UNO (unoken.astro@gmail.com) if
%%   you have a problem
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% useful command
\newcommand{\n}{\nonumber \\}
\newcommand{\p}{\partial}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\II}{I\negthinspace I}
\newcommand{\III}{I\negthinspace I\negthinspace I}
\newcommand{\mbm}[1]{\mbox{\protect \boldmath $#1$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  config for citation of figures, tables, and equations
%%%  to use English for all. 
%%%  2020.01.29 modified by Kentaro UNO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% figure and table
\captionsetup{compatibility=false}
%
\renewcommand{\figurename}{Fig.~\hspace{-.2em}}   
\renewcommand{\tablename}{Table~\hspace{-.2em}}

\captionsetup[figure]{format=plain,labelformat=simple,labelsep=colon,font=small}
\captionsetup[table]{format=plain,labelformat=simple,labelsep=colon,font=small}

\newcommand{\bhline}[1]{\noalign{\hrule height #1}} % bhlineコマンドの設定

%%% citation command for figures, tables, and equations
\newcommand{\fig}[1]{Fig.~\ref{#1}}
\newcommand{\subfig}[2]{Fig.~\ref{#1}\subref{#2}}
\newcommand{\fign}[1]{\ref{#1}}
\newcommand{\tb}[1]{Table~\ref{#1}}
\newcommand{\tabn}[1]{\ref{#1}}
\newcommand{\eq}[1]{Eq.~(\ref{#1})}
\newcommand{\eqn}[1]{(\ref{#1})}

%%% citation command for chapters, sections, and appendixes
\newcommand{\chap}[1]{Chap.~\ref{#1}}
\newcommand{\sect}[1]{Sect.~\ref{#1}}
\newcommand{\subsect}[1]{Sect.~\ref{#1}}
\newcommand{\app}[1]{Appnd. ~\ref{#1}}

%%% visualize a figure and table in a row
\makeatletter
\newcommand{\figcaption}[1]{\def\@captype{figure}\caption{#1}}
\newcommand{\tblcaption}[1]{\def\@captype{table}\caption{#1}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  ソースコードの引用スタイルの設定
%%%  2020.01.24 added by Kentaro UNO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{listings} %日本語のコメントアウトをする場合はjlistingが必要
%ここからソースコードの表示に関する設定
\definecolor{gray}{rgb}{0.9,0.9,0.9}
\lstset{
  backgroundcolor=\color{gray}, % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
  basicstyle={\small\ttfamily}, % the style of the fonts that are used for the code
  identifierstyle={\small}, % main()の''main''等のスタイル
  commentstyle={\small\itshape}, %//comment 等のスタイル
  keywordstyle={\small}, % int mainの''int''等のスタイル
  ndkeywordstyle={\small},
  stringstyle={\small\ttfamily},  % string literal style -> % printf(''Hello'')の''''で囲まれた部分のスタイル
  %frame={tb},
  breaklines=true, % sets automatic line breaking
  columns=[l]{fullflexible},
  numbers=left, % where to put the line-numbers; possible values are (none, left, right)
  numberstyle={\scriptsize}, % the style that is used for the line-numbers
  stepnumber=1, % the step between two line-numbers. If it's 1, each line will be numbered
  numbersep=1zw, % 行数字とコードの間のマージン
  xrightmargin=0zw, % 表示個所の右側マージン
  xleftmargin=2zw,  % 表示個所の左側マージン
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  lineskip=-0.5ex % codeの行間の設定
}

\def\epsgaiji#1{\leavevmode\kern-0.025zw\raise-.37zh\hbox{%
  \epsfile{file=#1,width=1.05zw}}\kern-0.025zw}
%\newcommand{\dfrac}[2]{\frac{\displaystyle{#1}}{\displaystyle{#2}}}
\newcommand{\MARU}[1]{{\ooalign{\hfil#1\/\hfil\crcr\raise.167ex\hbox{\mathhexbox20D}}}}

%%%
